Numerical methods for closed-loop systems with non-autonomous data

By computing a feedback control via the linear quadratic regulator (LQR) approach and simulating a non-linear non-autonomous closed-loop system using this feedback, we combine two numerically challenging tasks. For the first task, the computation of the feedback control, we use the non-autonomous generalized differential Riccati equation (DRE), whose solution determines the time-varying feedback gain matrix. Regarding the second task, we want to be able to simulate non-linear closed-loop systems for which it is known that the regulator is only valid for sufficiently small perturbations. Thus, one easily runs into numerical issues in the integrators when the closed-loop control varies greatly. For these systems, e.g., the A-stable implicit Euler methods fails.\newline On the one hand, we implement non-autonomous versions of splitting schemes and BDF methods for the solution of our non-autonomous DREs. These are well-established DRE solvers in the autonomous case. On the other hand, to tackle the numerical issues in the simulation of the non-linear closed-loop system, we apply a fractional-step-theta scheme with time-adaptivity tuned specifically to this kind of challenge. That is, we additionally base the time-adaptivity on the activity of the control. We compare this approach to the more classical error-based time-adaptivity.\newline We describe techniques to make these two tasks computable in a reasonable amount of time and are able to simulate closed-loop systems with strongly varying controls, while avoiding numerical issues. Our time-adaptivity approach requires fewer time steps than the error-based alternative and is more reliable.

==> bdf_algo/BDF_algo.tex <==
\IncMargin{1em}
\begin{algorithm}[t]
	\SetAlgoNoLine % no vertical lines for while/if/... 
	\KwIn{$\cA\time,\cM\time,\dot\cM\time,\cB\time,\cC\time,\weight,\timestepsbwd, \ord, L_0,\ldots,L_{\ord-1}, D_0,\ldots,D_{\ord-1}$}
	\KwOut{$\cK\kiterind, \kiter = 1,\ldots,\ntimestep$}
	\caption{Non-autonomous low-rank factor BDF method of order \ord{}}
	\label{algo:BDF}
	\BlankLine
	\For{$\kiter = \ord,\ldots,\ntimestep$}{\label{line:BDF1}
%	  $\timestep\kiterind = \tkhprev - \tkh$\label{line:BDF2}\;
	  $\cA\kiterind = \timestep\kiterind\beta\cA\timekh - \frac{1}{2}\cM\timekh$\label{line:BDF3}\;
	  $\cM\kiterind = \cM\timekh$\label{line:BDF4}\;
	  $\cB\kiterind = \sqrt{\timestep\beta}\cB\timekh$\label{line:BDF5}\;
	  $\cC\kiterind\transpose = \left[\cC\timekh\transpose, \cM\kiterind\transpose L_{\kiter - 1}, \ldots,
	  \cM\kiterind\transpose L_{\kiter - \ord}\right]$\label{line:BDF6}\;
	  $\cS\kiterind =  
	    \begin{blockmatrix}
	      \mblock(0,3)\timestep\beta I_\noutput(3,1)	\mblock(3,3)(4,1)				\mblock(7,3)(3,1)	\mblock(10,3)(3,1)
	      \mblock(0,2)(3,1)						\mblock(3,2)-\alpha_1 D_{\kiter - 1}(4,1)	\mblock(7,2)(3,1)	\mblock(10,2)(3,1)
	      \mblock(0,1)(3,1)						\mblock(3,1)(4,1)				\mblock(7,1)\ddots(1,1)	\mblock(10,1)(3,1)
	      \mblock(0,0)(3,1)						\mblock(3,0)(4,1)				\mblock(7,0)(3,1)	\mblock(10,0)-\alpha_{\ord}D_{\kiter - \ord}(3,1)
	    \end{blockmatrix}$\label{line:BDF7}\;
	  solve ARE \labelcref{eq:ARE} for $L\kiterind$ and $D\kiterind$ \label{line:BDF8}\;
	  $\cK\kiterindTbwd = \frac{1}{\sqrt{\weight}}\cB\timekh\transpose L\kiterindT D\kiterindT L\kiterind\transpose\cM\kiterind$\label{line:BDF9}\;
	  }
\end{algorithm}
\DecMargin{1em}

==> packages.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% packages
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage[utf8]{inputenc}
\usepackage{amsmath} % align
\usepackage{amsfonts}
\usepackage{amssymb}
\RequirePackage{graphicx}
\usepackage{subcaption}
\usepackage{tikz}
\usetikzlibrary{calc, positioning}
% \usetikzlibrary{shapes}
% \usetikzlibrary{shapes.misc} % for cross out
% \usepackage{pgfplots}
% \pgfplotsset{compat=1.13}

\usepackage{pgfplots}
\pgfplotsset{compat = 1.13,
%   colormap name = viridis,
  unbounded coords = jump,
%   every axis plot/.append style = {%
%     line width = 1.5pt
%   }
}
\tikzstyle{every node}=[font=\small]
\usepgfplotslibrary{external}
\tikzset{external/system call = {%
    lualatex \tikzexternalcheckshellescape
    -halt-on-error
    -interaction=batchmode
    -jobname "\image" "\texsource"}}
\tikzexternalize[prefix = tikz/externalize/]
\tikzexternaldisable{}
%\usepackage{subfig}
%\renewcommand{\thesubfigure}{Figure \arabic{subfigure}}
%\captionsetup[subfigure]{labelformat=simple, labelsep=colon}

\usepackage{filemod}
\newcommand{\includetikz}[1]{%
  \tikzexternalenable%
  \tikzsetnextfilename{#1}%
  \filemodCmp{tikz/#1.tikz}{tikz/externalize/#1.pdf}%
  {\tikzset{external/remake next}}{}%
  \input{tikz/#1.tikz}%
  \tikzexternaldisable%
}


% \usepackage[hidelinks]{hyperref}
% \usepackage[nameinlink,capitalise,noabbrev]{cleveref}
% \usepackage{mathrsfs} % curly capital letters
%\usepackage[ruled,linesnumbered]{algorithm2e} % algorithms
%\SetEndCharOfAlgoLine{}
% \usepackage{pgfplotstable}
\usepackage{xifthen}
\usepackage{mathrsfs} % curly capital letters

% algorithm2e keywords
%\SetKw{Not}{not}
%\SetKw{Or}{or}
%\SetKw{And}{and}

\RequirePackage[nameinlink,capitalise,noabbrev]{cleveref}
% labelcref has paranthesis for subequations
\crefalias{subequation}{equation}

\DeclareOldFontCommand{\rm}{\normalfont\rmfamily}{\mathrm}
\DeclareOldFontCommand{\sf}{\normalfont\sffamily}{\mathsf}
\DeclareOldFontCommand{\tt}{\normalfont\ttfamily}{\mathtt}
\DeclareOldFontCommand{\bf}{\normalfont\bfseries}{\mathbf}
\DeclareOldFontCommand{\it}{\normalfont\itshape}{\mathit}
\DeclareOldFontCommand{\sl}{\normalfont\slshape}{\@nomath\sl}
\DeclareOldFontCommand{\sc}{\normalfont\scshape}{\@nomath\sc}

\usepackage{doi}

%\setlength{\belowcaptionskip}{-1.8pt} % less space below figures
%\setlength{\floatsep}{20pt plus 2pt minus 2pt}


\usepackage[
% disable
]{todonotes}

\newcommand{\bjoern}[2][]{\todo[linecolor=magenta,size=\tiny,
backgroundcolor=magenta!25,bordercolor=magenta,#1]{BB: #2}}
\newcommand{\jens}[2][]{\todo[linecolor=black,size=\tiny,
backgroundcolor=black!25,bordercolor=black,#1]{JS: #2}}
\newcommand{\peter}[2][]{\todo[linecolor=blue,size=\tiny,
backgroundcolor=blue!25,bordercolor=blue,#1]{PB: #2}}
\newcommand{\tony}[2][]{\todo[linecolor=red,backgroundcolor=red!25,
bordercolor=red,size=\tiny,#1]{TS: #2}}
